Designing stellarators using perpendicular permanent magnets

We have developed a fast method to design perpendicular permanent magnets for simplifying stellarator coils based on existing codes. Coil complexity is one of the main challenges for stellarators. To date, only electromagnetic coils have been used to generate 3D fields for stellarators. Permanent magnets provide an alternative way to produce the desired magnetic field for optimized stellarators. In this paper, we revisit the concept of representing surface current using magnetic dipoles and carry out numerical validations. A surface magnetization is proven to be equivalent to the surface current that can be linearly solved by existing coil design codes. An incremental multi-layer method has been developed to obtain a practical solution that is attainable with present permanent magnets. With this method, we can reproduce a half-Tesla NCSX configuration using specially designed neodymium magnets together with simple planar coils. It shows that stellarator coils could be substantially simplified by adopting permanent magnets.

==> packages_commands.tex <==
 \usepackage{physics}
 \usepackage{hyperref}
 \usepackage{color}
 \usepackage{bm}
 \usepackage{graphicx, subcaption}
%\usepackage{adjustbox}
 \usepackage{latexsym}
 \usepackage{pifont}
 \usepackage{amssymb}
 \usepackage{hyperref}
 \usepackage{titlesec}
 \expandafter\let\csname equation*\endcsname\relax
 \expandafter\let\csname endequation*\endcsname\relax
 \usepackage{amsmath}
 \usepackage{listings}
 \usepackage{verbatim}
 \usepackage{geometry}
 \usepackage{booktabs}
 \usepackage{enumitem}
 \usepackage[normalem]{ulem} % for sout;
 \usepackage{breqn}
 \usepackage[toc,page]{appendix}
 
% COLORS
 \definecolor{red}{rgb}{1.0,0.0,0.0}
 \definecolor{gre}{rgb}{0.0,1.0,0.0}
 \definecolor{blu}{rgb}{0.0,0.0,1.0}

 \definecolor{ora}{rgb}{1.0,0.5,0.0}
 \definecolor{gra}{rgb}{0.0,0.5,1.0}

 \newcommand{\red}[1]{{\color{red} #1}}
 \newcommand{\gre}[1]{{\color{gre} #1}}
 \newcommand{\blu}[1]{{\color{red} #1}}  %color red

 \newcommand{\bro}[1]{{\color{bro} #1}}
 \newcommand{\gra}[1]{{\color{red} #1}}
 \newcommand{\ora}[1]{{\color{ora} #1}}

 \newcommand{\change}[2]{\sout{#1}\red{#2}}
 %\newcommand{\change}[2]{#2}
 \newcommand{\response}[2]{\sout{#1}\blu{#2}}
 %\newcommand{\response}[2]{#2}

% SHORT HAND 
 \newcommand{\ba}{\begin{abstract}}
 \newcommand{\ea}{\end{abstract}}
 \newcommand{\be}{\begin{equation}}
 \newcommand{\ee}{\end{equation}}

% \newcommand{\etal}{\textit{et al}. }
 \newcommand{\ie}{\textit{i}.\textit{e}., }
 \newcommand{\eg}{\textit{e}.\textit{g}. }

 \newcommand{\rom}[1]{\uppercase\expandafter{\romannumeral #1 \relax}}
 \newcommand{\Poincare}{Poincar$\acute{\rm e}$ }
 \newcommand{\iotabar}{\mbox{$\,\iota\!\!$-}}
 \newcommand{\Fig}[1]{Fig.\ref{fig:#1}}
 \newcommand{\Tab}[1]{Table.(\ref{tab:#1})}
 \newcommand{\Eqn}[1]{Eq.(\ref{eq:#1})}
 \newcommand{\Sec}[1]{Sec.\ref{sec:#1}}
 \renewcommand{\t}{\theta}
 \newcommand{\z}{\zeta} 
 \newcommand{\ds}{\displaystyle}
 
 \newcommand{\vect}[1]{\mathbf{#1}}
 %\newcommand{\dd}[1]{\textnormal{d} #1}
 %\newcommand{\pdv}[2]{\frac{\partial #1}{\partial #2}}
 %\newcommand{\dv}[2]{\frac{\dd{#1}}{\dd{#2}}}
 \newcommand{\hdv}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
 %\newcommand{\qty}{}
 %\newcommand{\abs}[1]{|#1|}
 %\newcommand{\grad}{\nabla}
 
 \newcommand{\bftab}{\fontseries{b}\selectfont}
 \newcommand{\half}{\frac{1}{2}}
 \newcommand{\tento}[1]{\times 10^{#1}}
